Where to Begin? On the Impact of Pre-Training and Initialization in Federated Learning

An oft-cited challenge of federated learning is the presence of heterogeneity. \emph{Data heterogeneity} refers to the fact that data from different clients may follow very different distributions. \emph{System heterogeneity} refers to the fact that client devices have different system capabilities. A considerable number of federated optimization methods address this challenge. In the literature, empirical evaluations usually start federated training from random initialization. However, in many practical applications of federated learning, the server has access to proxy data for the training task that can be used to pre-train a model before starting federated training. We empirically study the impact of starting from a pre-trained model in federated learning using four standard federated learning benchmark datasets. Unsurprisingly, starting from a pre-trained model reduces the training time required to reach a target error rate and enables the training of more accurate models (up to 40\%) than is possible when starting from random initialization. Surprisingly, we also find that starting federated learning from a pre-trained initialization reduces the effect of both data and system heterogeneity. We recommend that future work proposing and evaluating federated optimization methods evaluate the performance when starting from random and pre-trained initializations. We also believe this study raises several questions for further work on understanding the role of heterogeneity in federated optimization.

==> acks.tex <==
\section*{Acknowledgement}
We would like to thank Akshat Shrivastava, Hongyuan Zhan, Daniel Lazar, and Ashish Shenoy for their helpful discussions at various stages of this work.

==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}
\emph{Federated learning} (FL) has emerged as a popular distributed machine learning paradigm for privately training a shared model across many participants while the training data never leaves the participant devices. Our focus in this work is on understanding the impact of model initialization on federated learning.

In cross-device FL~\citep{fl-survey}, the primary setting considered in this paper, a large number of client devices (possibly on the order of hundreds of millions) participate in training, which is coordinated by a server. It is impractical for all devices to participate at every step of training; instead, FL usually proceeds in rounds and a small subset of available devices participate in each round. Each device possesses a local dataset, and the data at different devices follow different distributions, leading to the \emph{data heterogeneity} challenge~\citep{fl-survey}. Moreover, devices communicate with the server over low-bandwidth, high-latency links, making communication overhead a major performance factor.

The predominant approach to federated training builds on local update methods such as \textsc{FedAvg}~\citep{google-fedavg}, where a device performs several local updates (e.g., one epoch of SGD on their local training set) before transmitting an update to the server. Although this reduces communication overhead, it can also exacerbate the data heterogeneity problem. Several approaches have been proposed to address this challenge~\citep{fedprox,fedavgm,adaptive-fl-optimization,fednova,SCAFFOLD,karimireddy2021mime,zhang2021fedpd,acar2021feddyn}.

\textbf{This paper empirically investigates the impact of model initialization on federated optimization methods.} Previous empirical evaluations of FL methods nearly always start federated training from a randomly initialized model. Transfer learning from pre-trained models has become common practice in natural language processing~\cite{gpt2,devlin2018bert} and computer vision~\cite{he2019rethinking,vit}, yielding state-of-the-art results on many tasks and enabling faster model convergence in the centralized setting. However, the impact of starting federated training from a pre-trained model has not been carefully studied, even though in many practical applications of FL there is public proxy data available for pre-training at the server.

\paragraph{Contributions.} In this work we consider the question:
\begin{center}
    \it How does model initialization (random, or pre-trained) impact \\the behavior of federated optimization methods?
\end{center}
Towards answering this question, we perform an extensive empirical study, comparing 15 variations of federated optimization methods on four commonly-used FL benchmark datasets. Our study reveals four key findings:
\begin{enumerate}
    % \item Federated optimization methods behave differently when initialized randomly versus from pre-trained weights (Section~\ref{sec:results_ranking}). \mike{Definitely rewrite this to be more specific; currently too vague or just not so surprising.}
    % \item \mike{Shouldn't the first point be about optimizers designed to address heterogeneity not being the best when starting from a pre-trained initialization?}
    \item Optimizers designed to address heterogeneity are not as effective when starting from pre-trained initialization. 
    % the effect of system and data heterogeneity is less of a problem when initializing federated optimization from a pre-trained solution.  \mike{Again, elaborate on exactly what ``less of a problem'' means here.}

    \item Starting from a pre-trained solution can close the gap between training on IID and non-IID data (Section~\ref{sec:results}). Moreover, the simple \sgd at the client outperforms more complex local-update methods in the pre-trained setting.
    
    \item Towards starting to explain this phenomenon, we observe that inter-device gradient/update diversity is higher for random initialized model at the beginning of training, and inter-device cosine similarity is higher when starting from a pre-trained model. (Section~\ref{sec:why_pretrain})
    
    \item When starting from a pre-trained solution, the client can afford to take more local steps to save on communications without hurting final accuracy. \john{Reword this finding}
    
    % Surprisingly, full-batch gradient descent, without any local steps, achieves performance competitive with other SoTA local-update methods from a pre-trained initialization. 

    % \mike{Maybe add something specifically about the performance of local-update methods vs those that don't use local updates (FedGD, ...)?}

\end{enumerate}
Our experiments also confirm what one might expect, that initializing FL with a pre-trained model can increase final model accuracy and reduce the number of rounds required to achieve a target accuracy, thereby saving communications and reducing the overall training time. This is evident in Figure~1 across several datasets (hyperparameters were tuned separately for each dataset--initialization pair; see Section~\ref{sec:experiments} for details of the experimental setup). 

\begin{figure*}[t]
     \centering
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_pre_ran.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_charlm_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/reddit_ran_pre.pdf}
     \end{minipage}
      \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_resnet_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_resnet_ran_pre.pdf}
     \end{minipage}
     \caption{While prior works ignore the importance of initialization, using pre-trained models should be the first step for any practical deployment to save on communication bandwidth and achieve high model accuracy. This figure shows the advantage of using a pre-trained model for four tasks. For Stack Overflow and Reddit, we use DistilGPT2 and CharLM. For CIFAR-10 and FEMNIST, we use SqueezeNet and ResNet18. }
     \label{fig:pretrained_vs_random}
\end{figure*}

Our findings are reproducible using the open-source federated learning framework FLSim~\cite{flsim}. Informed by these findings, we conclude by presenting several recommendations for future research on federated optimization.
